Fast 3D Synthetic Aperture Radar Imaging from Polarization-Diverse Measurements

An innovative 3-D radar imaging technique is developed for fast and efficient identification and characterization of radar backscattering components of complex objects, when the collected scattered field is made of polarization-diverse measurements. In this context, all the polarimetric information seems irretrievably mixed. A direct model, derived from a simple but original extension of the widespread "multiple scattering model" leads to a high dimensional linear inverse problem. It is solved by a fast dedicated imaging algorithm that performs to determine at a time three huge 3-D scatterer maps which correspond to HH, VV and HV polarizations at emission and reception. It is applied successfully to various mock-ups and data sets collected from an accurate and dedicated 3D spherical experimental layout that provides concentric polarization-diverse RCS measurements.

==> abrege.tex <==
% TEX 7(ascii) bits
%
% ABREGE.tex
% LaTeX document
% Author: J.I. 
% Date  : Juillet 1996
%
% Raccourcis d'expressions très usitées
%
% Derniere modif le 10-07-96
%
%
% ==> OK, JFG -- 26/04/2010
%

% Raccourci pour \XS
\def\XS{\xspace}

%%%%%%%%%%%%%%%%%%% Pour definir nouvelle commande de changement de taille
\RequirePackage{ifthen}
\RequirePackage{calc}

\newcommand{\taille}[1][\scad]{%
\ifthenelse{#1 = -5}{}{}%
\ifthenelse{#1 = -4}{\tiny}{}%
\ifthenelse{#1 = -3}{\scriptsize}{}%
\ifthenelse{#1 = -2}{\footnotesize}{}%
\ifthenelse{#1 = -1}{\small}{}%
\ifthenelse{#1 = 0}{\normalsize}{}%
\ifthenelse{#1 = 1}{\large}{}%
\ifthenelse{#1 = 2}{\Large}{}%
\ifthenelse{#1 = 3}{\LARGE}{}%
\ifthenelse{#1 = 4}{\huge}{}%
\ifthenelse{#1 = 5}{\Huge}{}}

\newboolean{@serif}
\setboolean{@serif}{true}
\def\scad{-5} % scadefaultsize

\newcounter{taille}
\newcommand{\sca}[2][\scad]{\setcounter{taille}{#1}%
  \ifthenelse{\boolean{@serif}}
  {{\taille[\thetaille]\textsc{#2}}}
  {\setcounter{taille}{\value{taille}-1}{\uppercase{\taille[\thetaille]#2}}}}


%%% RACCOURCIS DIVERS %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

% Mise en commentaire rapide !
	\def\Rem#1{}                    % rem{bla bla bla}

% References automatiquement entre parenthese
	%\def\reff#1{\XS(\ref{#1})}
	%\def\refs#1{section~\ref{#1}}
	%\def\refS#1{Section~\ref{#1}}

% Nettoyage
	%\newcommand{\clearemptydoublepage}{\newpage{\pagestyle{empty}\cleardoublepage}}  

% Numéro (pour biblio)
	\def\numero{n°}
	\def\Numero{N°}

% Majuscules
	\def\UP#1{\uppercase{#1}}       % majuscules
	\def\up#1{\uppercase{#1}}       % majuscules

% References automatiquement entre parenthese
 \def\reff#1{\XS(\ref{#1})}
 %\def\refs#1{section~\ref{#1}}
 %\def\refS#1{Section~\ref{#1}}

%%% RACCOURCIS d'italique, locutions,... %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\def\adhoc{\textit{ad hoc}\XS}
\def\apost{\textit{a posteriori}\XS}
\def\Apost{\textit{A posteriori}\XS}
\def\APost{\textit{A Posteriori}\XS}
\def\post{\textit{posterior}\XS}
\def\Post{\textit{Posterior}\XS}
\def\afortio{\textit{a fortiori}\XS}
\def\Afortio{\textit{A fortiori}\XS}
\def\aprio{\textit{a priori}\XS}
\def\Aprio{\textit{A priori}\XS}
\def\Cad{C'est-à-dire\XS}
\def\cad{c'est-à-dire\XS}
\def\Cpq{C'est pourquoi\XS}
\def\cpq{c'est pourquoi\XS}
\def\coeur{c{\oe}ur\XS}
\def\cf{\textit{cf.}\XS}
\def\eg{\textit{e.g.,}\XS}
\def\etal{\textit{et al.}\XS}
\def\etc{\textit{etc\dots}\XS}
\def\etcoll{{\textit et coll.}\XS}
\def\idem{\textit{idem}\XS}
\def\ie{\textit{i.e.,}\XS}
\def\iid{i.i.d.\XS}
\def\infine{\textit{in fine}\XS}
\def\insit{\textit{in situ}\XS}
\def\inviv{\textit{in vivo}\XS}
\def\oeuvre{{\oe}uvre\XS}
\def\oeuvres{{\oe}uvres\XS}
\def\oeil{{\oe}il\XS}
\def\recto{\textit{recto}\XS}
\def\Toeplitz{T{\oe}plitz\XS}
\def\vav{vis-à-vis\XS}
\def\via{\textit{via}\XS}
\def\vic{\textit{vice-versa}\XS}
\def\verso{\textit{verso}\XS}
\def\vs{\textit{vs}\XS}
\def\versus{\textit{versus}\XS}
\def\ssi{\textit{si et seulement si}\XS}
\def\strsen{\textit{stricto sensu}\XS}
\def\wrt{w.r.t.\XS}

\def\ier{$^{\text{\small er}}$\XS}
\def\iere{$^{\text{\small re}}$\XS}
\def\ieme{$^{\text{\small e}}$\XS}

\def\primo{\ensuremath{1^{\oD}}\XS}
\def\secundo{\ensuremath{2^{\oD}}\XS}
\def\tertio{\ensuremath{3^{\oD}}\XS}
\def\quatro{\ensuremath{4^{\oD}}\XS}

	\def\MALDI{Matrix-Assisted Laser Desorption/Ionisation\XS}
	\newcommand{\maldi}[1][\scad]{\sca[#1]{maldi}\XS}

	\def\BHIPRO{Bayesian Hierarchical Inversion in Proteomics\XS}
	\newcommand{\bhipro}[1][\scad]{\sca[#1]{bhi-pro}\XS}


%%% ACRONYMES %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

% Divers 
	\newcommand{\art}[1][\scad]{\sca[#1]{art}\XS}
	\newcommand{\cnd}[1][\scad]{\sca[#1]{cnd}\XS}
	\newcommand{\ndt}[1][\scad]{\sca[#1]{ndt}\XS}
	\newcommand{\gnc}[1][\scad]{\sca[#1]{gnc}\XS}
	\newcommand{\mfa}[1][\scad]{\sca[#1]{mfa}\XS}
	\newcommand{\map}[1][\scad]{\sca[#1]{map}\XS}

	\newcommand{\icm}[1][\scad]{\sca[#1]{icm}\XS}
	\newcommand{\icd}[1][\scad]{\sca[#1]{icd}\XS}
	\newcommand{\rsb}[1][\scad]{\sca[#1]{rsb}\XS}
	\newcommand{\snr}[1][\scad]{\sca[#1]{snr}\XS}
	\newcommand{\fft}[1][\scad]{\sca[#1]{fft}\XS}
	\newcommand{\fftdd}[1][\scad]{\sca[#1]{fft-2d}\XS}
	\newcommand{\ifft}[1][\scad]{\sca[#1]{ifft}\XS}
	\newcommand{\dsp}[1][\scad]{\sca[#1]{dsp}\XS}

	\newcommand{\dess}[1][\scad]{\sca[#1]{dess}\XS}
	\newcommand{\dea}[1][\scad]{\sca[#1]{dea}\XS}
	\newcommand{\deug}[1][\scad]{\sca[#1]{deug}\XS}
	\newcommand{\deust}[1][\scad]{\sca[#1]{deust}\XS}
	\newcommand{\iut}[1][\scad]{\sca[#1]{iut}\XS}
	\newcommand{\iup}[1][\scad]{\sca[#1]{iup}\XS}
	\newcommand{\ects}[1][\scad]{\sca[#1]{ects}\XS}

	\newcommand{\ufr}[1][\scad]{\sca[#1]{ufr}\XS}
   \newcommand{\upr}[1][\scad]{\sca[#1]{upr}\XS}

	\newcommand{\gbm}[1][\scad]{\sca[#1]{gbm}\XS}
	\newcommand{\irmf}[1][\scad]{\sca[#1]{irm-f}\XS}
	\newcommand{\irm}[1][\scad]{\sca[#1]{irm}\XS}
	\newcommand{\rmn}[1][\scad]{\sca[#1]{rmn}\XS}
	\newcommand{\eeg}[1][\scad]{\sca[#1]{eeg}\XS}
	\newcommand{\meg}[1][\scad]{\sca[#1]{meg}\XS}


% Transformées
	\newcommand{\tf}[1][\scad]{\sca[#1]{tf}\XS}
	%\newcommand{\sf}[1][\scad]{\sca[#1]{sf}\XS}
	\def\sf{\textsc{sf}\XS}
	\newcommand{\tl}[1][\scad]{\sca[#1]{tl}\XS}
	\newcommand{\tz}[1][\scad]{\sca[#1]{tz}\XS}
	\newcommand{\tpsc}[1][\scad]{\sca[#1]{tc}\XS}
	\newcommand{\tpsd}[1][\scad]{\sca[#1]{td}\XS}

% Operating Systemes 
	\newcommand{\linux}[1][\scad]{\sca[#1]{Linux}\XS}
	\newcommand{\unix}[1][\scad]{\sca[#1]{Unix}\XS}
	\newcommand{\msdos}[1][\scad]{\sca[#1]{msdos}\XS}
	\newcommand{\sunos}[1][\scad]{\sca[#1]{Sunos}\XS}
	\newcommand{\hupux}[1][\scad]{\sca[#1]{hp-ux}\XS}
	\newcommand{\vms}[1][\scad]{\sca[#1]{vms}\XS}
	\newcommand{\solaris}[1][\scad]{\sca[#1]{Solaris}\XS}
	\newcommand{\winnt}[1][\scad]{\sca[#1]{Windows-nt}\XS}
	\newcommand{\vmware}[1][\scad]{\sca[#1]{vmware}\XS}
	\newcommand{\win}[1][\scad]{\sca[#1]{Windows}\XS}

% Calcul scientifique
	\newcommand{\labview}[1][\scad]{\sca[#1]{Labview}\XS}
	\newcommand{\matlab}[1][\scad]{\sca[#1]{Matlab}\XS}
	\newcommand{\maple}[1][\scad]{\sca[#1]{Maple}\XS}
	\newcommand{\mathe}[1][\scad]{\sca[#1]{Mathematica}\XS}
	\newcommand{\idl}[1][\scad]{\sca[#1]{Idl}\XS}

% Langages
	\newcommand{\cmex}[1][\scad]{\sca[#1]{Cmex}\XS}
	\newcommand{\pascal}[1][\scad]{\sca[#1]{Pascal}\XS}
	\newcommand{\java}[1][\scad]{\sca[#1]{Java}\XS}
	\newcommand{\lisp}[1][\scad]{\sca[#1]{Lisp}\XS}
	\newcommand{\forts}[1][\scad]{\sca[#1]{Fortran}{\footnotesize 77}\XS}
	\newcommand{\fortq}[1][\scad]{\sca[#1]{Fortran}{\footnotesize 90}\XS}
	\newcommand{\ada}[1][\scad]{\sca[#1]{Ada}\XS}
	\newcommand{\eiffel}[1][\scad]{\sca[#1]{Eiffel}\XS}
	\newcommand{\tcsh}[1][\scad]{\sca[#1]{tcsh}\XS}
	\newcommand{\bash}[1][\scad]{\sca[#1]{bash}\XS}
	\newcommand{\lgc}[1][\scad]{\sca[#1]{C}\XS}
	\newcommand{\cpp}[1][\scad]{\sca[#1]{C}{\footnotesize ++}\XS}

% Congres
	\newcommand{\gretsi}[1][\scad]{\sca[#1]{gretsi}\XS}
	\newcommand{\maxent}[1][\scad]{\sca[#1]{maxent}\XS}
	\newcommand{\icip}[1][\scad]{\sca[#1]{icip}\XS}
	\newcommand{\icassp}[1][\scad]{\sca[#1]{icassp}\XS}
	\newcommand{\spie}[1][\scad]{\sca[#1]{spie}\XS}
	\newcommand{\gdr}[1][\scad]{\sca[#1]{gdr--prc~isis}\XS}
	\newcommand{\rfia}[1][\scad]{\sca[#1]{rfia}\XS}
	\newcommand{\eusipco}[1][\scad]{\sca[#1]{eusipco}\XS}

% Restes
	\newcommand{\leti}[1][\scad]{\sca[#1]{leti}\XS}
	\newcommand{\cesta}[1][\scad]{\sca[#1]{cesta}\XS}
	\newcommand{\minatec}[1][\scad]{\sca[#1]{minatec}\XS}
	\newcommand{\stic}[1][\scad]{\sca[#1]{stic}\XS}
	\newcommand{\pc}[1][\scad]{\sca[#1]{pc}\XS}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% Ajout de famouss.tex
% modif le 25/5/2000 Phiphi
% GPInuts - Famous people - VIP
%
\newcommand{\beaunom}[4][0]{{\taille[#1]#2 \uppercase{#3}}%
{\sca[#1]{#4}}\XS}

%\newcommand{\MA}[1][\scad]{{\taille[#1]Marc \uppercase{A}}% 
%{\sca[#1]{llain}\XS}}
\newcommand{\AuGi}[1][\scad]{\beaunom[#1]{Audrey}{G}{iremus}}

\newcommand{\AB}[1][\scad]{\beaunom[#1]{Amandine}{B}{lanc}}
\newcommand{\ABF}[1][\scad]{\beaunom[#1]{Amandine}{B}{lanc~--~Fusco}}
\newcommand{\AAB}[1][\scad]{\beaunom[#1]{Alain}{A}{bergel}}
\newcommand{\AC}[1][\scad]{\beaunom[#1]{Alain}{C}{oulais}}
\newcommand{\AH}[1][\scad]{\beaunom[#1]{Alain}{H}{erment}}
\newcommand{\AG}[1][\scad]{\beaunom[#1]{Audrey}{G}{iremus}}
\newcommand{\AHz}[1][\scad]{\beaunom[#1]{Aurélien}{H}{azart}}
\newcommand{\AMD}[1][\scad]{\beaunom[#1]{Ali}{M}{ohammad--Djafari}}
\newcommand{\AR}[1][\scad]{\beaunom[#1]{Andrea}{R}{idolfi}}
\newcommand{\BDuc}[1][\scad]{\beaunom[#1]{Bernard}{D}{uchêne}}
\newcommand{\CH}[1][\scad]{\beaunom[#1]{Christian}{H}{einrich}}
\newcommand{\CS}[1][\scad]{\beaunom[#1]{Charles}{S}{oussen}}
\newcommand{\CV}[1][\scad]{\beaunom[#1]{Cornelia}{V}{acar}}
\newcommand{\DLB}[1][\scad]{\beaunom[#1]{Denis}{L}{e Bihan}}
\newcommand{\FA}[1][\scad]{\beaunom[#1]{Frédéric}{A}{uchère}}
\newcommand{\FC}[1][\scad]{\beaunom[#1]{Frédéric}{C}{hampagnat}}
\newcommand{\FL}[1][\scad]{\beaunom[#1]{Franck}{L}{etimonier}}
\newcommand{\FV}[1][\scad]{\beaunom[#1]{Francisco}{V}{arela}}
\newcommand{\FDU}[1][\scad]{\beaunom[#1]{Frédéric}{D}{ublanchet}}
\newcommand{\FB}[1][\scad]{\beaunom[#1]{François}{B}{oulanger}}
\newcommand{\FO}[1][\scad]{\beaunom[#1]{Fran\c{c}ois}{O}{rieux}}
\newcommand{\GDE}[1][\scad]{\beaunom[#1]{Guy}{D}{emoment}}
\newcommand{\GS}[1][\scad]{\beaunom[#1]{Grégory}{S}{trubel}}
\newcommand{\GLB}[1][\scad]{\beaunom[#1]{Guy}{L}{e Besnerais}}
\newcommand{\GL}[1][\scad]{\beaunom[#1]{Guilaine }{L}{agache}}
\newcommand{\GR}[1][\scad]{\beaunom[#1]{Gilles}{R}{ochefort}}
\newcommand{\HC}[1][\scad]{\beaunom[#1]{Hervé}{C}{arfantan}}
\newcommand{\HS}[1][\scad]{\beaunom[#1]{Hichem}{S}{noussi}}
\newcommand{\JCV}[1][\scad]{\beaunom[#1]{Jean--Claude}{V}{ial}}
\newcommand{\JFB}[1][\scad]{\beaunom[#1]{Jean--Fran\c{c}ois}{B}{ercher}}
\newcommand{\JFG}[1][\scad]{\beaunom[#1]{Jean\,--\,Fran\c{c}ois}{G}{iovannelli}}
\newcommand{\JFM}[1][\scad]{\beaunom[#1]{Jean--Fran\c{c}ois}{M}{angin}}
\newcommand{\JI}[1][\scad]{\beaunom[#1]{Jérôme}{I}{dier}}
\newcommand{\JBP}[1][\scad]{\beaunom[#1]{Jean-Baptiste}{P}{oline}}
\newcommand{\KS}[1][\scad]{\beaunom[#1]{Ken}{S}{auer}}
\newcommand{\LG}[1][\scad]{\beaunom[#1]{Line}{G}{arnero}}
\newcommand{\MA}[1][\scad]{\beaunom[#1]{Marc}{A}{llain}}
\newcommand{\MF}[1][\scad]{\beaunom[#1]{Marc}{F}{ayolle}}
\newcommand{\Mimi}[1][\scad]{\beaunom[#1]{Myriam}{F}{iani}}
\newcommand{\MN}[1][\scad]{\beaunom[#1]{Mila}{N}{ikolova}}
\newcommand{\NBA}[1][\scad]{\beaunom[#1]{Nicolas}{B}{arbey}}
\newcommand{\OF}[1][\scad]{\beaunom[#1]{Olivier}{F}{\'eron}}
\newcommand{\PC}[1][\scad]{\beaunom[#1]{Philippe}{C}{iuciu}}
\newcommand{\PG}[1][\scad]{\beaunom[#1]{Pierre}{G}{rangeat}}
\newcommand{\PS}[1][\scad]{\beaunom[#1]{Pascal}{S}{zacherski}}
\newcommand{\RB}[1][\scad]{\beaunom[#1]{Redha}{B}{oubertakh}}
\newcommand{\SB}[1][\scad]{\beaunom[#1]{Stéphane}{B}{rette}}
\newcommand{\SG}[1][\scad]{\beaunom[#1]{Stéphane}{G}{autier}}
\newcommand{\SBA}[1][\scad]{\beaunom[#1]{Sylvain}{B}{ailet}}
\newcommand{\TM}[1][\scad]{\beaunom[#1]{Thierry}{M}{artin}}
\newcommand{\TR}[1][\scad]{\beaunom[#1]{Thomas}{R}{odet}}
\newcommand{\VS}[1][\scad]{\beaunom[#1]{Vincent}{S}{amson}}
\newcommand{\YB}[1][\scad]{\beaunom[#1]{Yannick}{B}{erthoumieu}}
\newcommand{\YG}[1][\scad]{\beaunom[#1]{Yves}{G}{oussard}}



% Acronymes et raccourcis

	\def\EEA{Électronique Électrotechnique Automatique\XS}
	\newcommand{\eea}[1][\scad]{\sca[#1]{eea}\XS}

	\def\ANR{Agence Nationale de la Recherche\XS}
	\newcommand{\anr}[1][\scad]{\sca[#1]{anr}\XS}

	\def\ENSEIRB{École Nationale Supérieure d'\'Electronique, Informatique et Télécommunications de Bordeaux\XS}
	\newcommand{\enseirb}[1][\scad]{\sca[#1]{enseirb}\XS}

	\def\ENSC{École Nationale Supérieure de Cognitique\XS}
	\newcommand{\ensc}[1][\scad]{\sca[#1]{ensc}\XS}

	\def\ATS{Automatique et Traitement du Signal\XS}
	\newcommand{\ats}[1][\scad]{\sca[#1]{ats}\XS}

	\def\THCS{Traitement Harmonique et Contrôle du Signal\XS}
	\newcommand{\thcs}[1][\scad]{\sca[#1]{thcs}\XS}

	\def\TE{travaux d'études\XS}
	\newcommand{\te}[1][\scad]{\sca[#1]{te}\XS}

	\def\TD{travaux dirigés\XS}
	\def\GTD{Travaux dirigés\XS}
	\newcommand{\td}[1][\scad]{\sca[#1]{td}\XS}

	\def\TP{travaux pratiques\XS}
	\def\GTP{Travaux pratiques\XS}
	\newcommand{\tp}[1][\scad]{\sca[#1]{tp}\XS}

	\def\TDAO{travaux dirigés assistés sur ordinateur\XS}
	\newcommand{\tdao}[1][\scad]{\sca[#1]{tdao}\XS}

	\def\ATER{Attaché temporaire d'enseignement et de recherche}
	\newcommand{\ater}[1][\scad]{\sca[#1]{ater}\xspace}

	\def\ADDOC{Agir pour les Doctorants et les jeunes Docteurs\XS}
	\newcommand{\addoc}[1][\scad]{\sca[#1]{addoc}\XS}

	\def\SHFJ{Service Hospitalier Frédéric Joliot\XS}
	\newcommand{\shfj}[1][\scad]{\sca[#1]{shfj}\XS}

	\def\UNAF{Unité de Neuroimagerie Anatomo Fonctionnelle\XS}
	\newcommand{\unaf}[1][\scad]{\sca[#1]{unaf}\XS}

	\def\CHU{Centre Hospitalier Universitaire\XS}
	\newcommand{\chu}[1][\scad]{\sca[#1]{chu}\XS}

	\def\LIF{Laboratoire d'Imagerie Fonctionnelle\XS}
	\newcommand{\lif}[1][\scad]{\sca[#1]{lif}\XS}

	\def\CEA{Commissariat à l'Énegie Atomique\XS}
	\newcommand{\cea}[1][\scad]{\sca[#1]{cea}\XS}

	\def\DRM{Département de Recherche Médicale\XS}
	\newcommand{\drm}[1][\scad]{\sca[#1]{drm}\XS}

	\def\DAM{Direction des Affaires Militaires\XS}
	\newcommand{\dam}[1][\scad]{\sca[#1]{dam}\XS}

	\def\DSV{Direction des Sciences du Vivant\XS}
	\newcommand{\dsv}[1][\scad]{\sca[#1]{dsv}\XS}

	\def\CNRS{Centre National de la Recherche Scientifique\XS}
	\newcommand{\cnrs}[1][\scad]{\sca[#1]{cnrs}\XS}

	\def\UMR{Unité Mixte de Recherche\XS}
	\newcommand{\umr}[1][\scad]{\sca[#1]{umr}\XS}

	\def\CNES{Centre National d'Études Spatiales\XS}
	\newcommand{\cnes}[1][\scad]{\sca[#1]{cnes}\XS}

	\def\EDF{Électricité de France\XS}
	\newcommand{\edf}[1][\scad]{\sca[#1]{edf}\XS}

	\def\ENSTA{École Nationale Supérieure de Techniques Avancées\XS}
	\newcommand{\ensta}[1][\scad]{\sca[#1]{ensta}\XS}

	\def\ENST{École Nationale Supérieure des Télécommunications\XS}
	\newcommand{\enst}[1][\scad]{\sca[#1]{enst}\XS}

	\def\ESIEA{École Supérieure d'Informatique Électronique Automatique\XS}
	\newcommand{\esiea}[1][\scad]{\sca[#1]{esiea}\XS}

	\def\ENSEA{École Nationale Supérieure de l'Électronique et des ses Applications\XS}
	\newcommand{\ensea}[1][\scad]{\sca[#1]{ensea}\XS}

	\def\GPI{Groupe Problèmes Inverses\XS}
	\newcommand{\gpi}[1][\scad]{\sca[#1]{gpi}\XS}

	\def\GSI{Groupe Signal~--~Image\XS}
	\newcommand{\gsi}[1][\scad]{\sca[#1]{gsi}\XS}

	\def\IPB{Institut Polytechnique de Bordeaux\XS}
	\newcommand{\ipb}[1][\scad]{\sca[#1]{ipb}\XS}

	\def\INSERM{Institut National pour la Santé et la Recherche Médicale\XS}
	\newcommand{\inserm}[1][\scad]{\sca[#1]{inserm}\XS}

	\def\CNAM{Conservatoire National des Arts et Métiers\XS}
	\newcommand{\cnam}[1][\scad]{\sca[#1]{cnam}\XS}

	\def\OPM{Observatoire de Paris\XS}
	\newcommand{\opm}[1][\scad]{\sca[#1]{opm}\XS}

	\def\INRIA{Institut National de Recherche et Informatique et Automatique\XS}
	\newcommand{\inria}[1][\scad]{\sca[#1]{inria}\XS}

	\def\IAS{Institut d'Astrophysique Spatiale\XS}
	\newcommand{\ias}[1][\scad]{\sca[#1]{ias}\XS}

	\def\IAP{Institut d'Astrophysique de Paris\XS}
	\newcommand{\iap}[1][\scad]{\sca[#1]{iap}\XS}

	\def\IPSN{Institut de Protection et de Sureté Nucléaire\XS}
	\newcommand{\ipsn}[1][\scad]{\sca[#1]{ipsn}\XS}

	\def\LSS{Laboratoire des Signaux et Systèmes\XS}
	\newcommand{\lss}[1][\scad]{\sca[#1]{lss}\XS}

	\def\LAPS{Laboratoire Automatique, productique, Signal\XS}
	\newcommand{\laps}[1][\scad]{\sca[#1]{laps}\XS}

	\def\LIMS{Laboratoire de l'Int\'egration du Mat\'eriau au Syst\`eme\XS}
	\def\IMS{Int\'egration du Mat\'eriau au Syst\`eme\XS}
	\newcommand{\ims}[1][\scad]{\sca[#1]{ims}\XS}

	\def\IMB{Institut de Mathématique de Bordeaux\XS}
	\newcommand{\imb}[1][\scad]{\sca[#1]{imb}\XS}

	\def\LaBRI{Laboratoire Bordelais de Recherche en Informatique\XS}
	\newcommand{\labri}[1][\scad]{\sca[#1]{labri}\XS}

	\def\LIMSI{Laboratoire d'Informatique pour la Mécanique et les Sciences de l'Ingénieur\XS}
	\newcommand{\limsi}[1][\scad]{\sca[#1]{limsi-cnrs}\XS}

	\def\ONERA{Office National d'Études et de Recherches Aérospatiales\XS}
	\newcommand{\onera}[1][\scad]{\sca[#1]{onéra}\XS}

	\def\CLS{Collecte Localisation Satellites\XS}
	\newcommand{\cls}[1][\scad]{\sca[#1]{cls}\XS}

	\def\SSL{signaux et systèmes linéaires\XS}
	\def\GSSL{Signaux et systèmes linéaires\XS}
	\newcommand{\ssl}[1][\scad]{\sca[#1]{ssl}\XS}

	\def\IFIPS{Institut de Formation des Ingénieurs de Paris-Sud\XS}
	\newcommand{\ifips}[1][\scad]{\sca[#1]{ifips}\XS}

	\def\IST{Information, Systèmes et Technologie\XS}
	\newcommand{\isp}[1][\scad]{\sca[#1]{ist}\XS}

	\def\LMD{Licence, Master, Doctorat\XS}
	\newcommand{\lmd}[1][\scad]{\sca[#1]{lmd}\XS}

   \def\MDC{Maître de conférences\XS}
   \newcommand{\mdc}[1][\scad]{\sca[#1]{mdc}\XS}

   \def\UPS{Université Paris-Sud\XS}
   \newcommand{\ups}[1][\scad]{\sca[#1]{ups}\XS}

   \def\UBI{Universit\'e Bordeaux~1\XS}
   \newcommand{\ubI}[1][\scad]{\sca[#1]{ub{\footnotesize 1}}\XS}

   \def\UdB{Universit\'e de Bordeaux\XS}
   \newcommand{\udb}[1][\scad]{\sca[#1]{ub}\XS}



% Unites Thomson
   %\newcommand{\thomair}[1][\scad]{\sca[#1]{Thomson-csf Airsys}\XS}
   %\newcommand{\oscar}[1][\scad]{\sca[#1]{Oscar}\XS}
   %\newcommand{\thomrcm}[1][\scad]{\sca[#1]{Thomson-rcm}\XS}

% Divers à virer...
   % LENA, lena upr640,...
   %\newcommand{\uprlen}[1][\scad]{\sca[#1]{upr}{\footnotesize 640}\XS}
   %\def\LENA{Laboratoire d'Encéphalographie et de Neurophysiologie Appliquée\XS}
   %\newcommand{\lena}[1][\scad]{\sca[#1]{lena}\XS}

   %\newcommand{\UFRPhys}[1][\scad]{{\ufr de physique}\XS}
   %\newcommand{\ups}[1][\scad]{\sca[#1]{ups}\XS}




==> alphabet.tex <==
% Document LaTeX        Auteur : Guy Le Besnerais       Date : 25/05/94
% Modification : J.-F. Gio      (15/09/95)
%                               J.I. (format Latex 2e, taille adaptative 22/03/99)
%                                    (fonte blackboard 27/08/99)
%
% ==> OK, JFG -- 26/04/2010
%
% Objet : Definitions compactes d'alphabets pour ecriture en Math
% b pour bold italique : \Ab
% v pour bold droit : \Av
% D pour droit : \AD
% c pour cursif : \Ac
% bb pour blackboard : \Abb
% Capitale pour capitale : \Lambda

\typeout{\space}
\typeout{\space\space\space\space Fichier 'alphabet.tex' -- LSS 1994/95/99}
\typeout{\space\space\space\space (necessite les packages xspace, amsmath, bbm)}
\typeout{\space}

\RequirePackage{amsmath}
\RequirePackage{xspace}
%\RequirePackage{bbm}
\RequirePackage{dsfont}
\RequirePackage{oldgerm}		% 04.06.2003   Pour les alphabet Gothiques

%-------------------------------------------

% DEFINITIONS PRELIMINAIRES 

\def\XS{\xspace}
\DeclareMathAlphabet{\mathb}{OML}{cmm}{b}{it}
\def\sbm#1{\ensuremath{\mathb{#1}}}                % Style gras italique (necessite amsmath)           
%
\def\sbmm#1{\ensuremath{\boldsymbol{#1}}}          % Style gras italique (necessite amsmath)           
\def\sdm#1{\ensuremath{\mathrm{#1}}}               % Style droit en math
\def\sbv#1{\ensuremath{\mathbf{#1}}}               % Style gras droit
\def\scu#1{\ensuremath{\mathcal{#1\XS}}}           % Style cursif
\def\scb#1{\ensuremath{\boldsymbol{\mathcal{#1}}}} % Style gras cursif

%\def\sbl#1{\ensuremath{\mathbbm{#1}}}              % Style blackboard (necessite bbm)
\def\sbl#1{\ensuremath{\mathds{#1}}}              % Style blackboard (necessite bbm)

%-------------------------------------------

% ALPHABET GRAS ITALIQUE, taille adaptative

\def\Ab{{\sbm{A}}\XS}  \def\ab{{\sbm{a}}\XS}
\def\Bb{{\sbm{B}}\XS}  \def\bb{{\sbm{b}}\XS}
\def\Cb{{\sbm{C}}\XS}  \def\cb{{\sbm{c}}\XS}
\def\Db{{\sbm{D}}\XS}  \def\db{{\sbm{d}}\XS}
\def\Eb{{\sbm{E}}\XS}  \def\eb{{\sbm{e}}\XS}
\def\Fb{{\sbm{F}}\XS}  \def\fb{{\sbm{f}}\XS}
\def\Gb{{\sbm{G}}\XS}  \def\gb{{\sbm{g}}\XS}
\def\Hb{{\sbm{H}}\XS}  \def\hb{{\sbm{h}}\XS}
\def\Ib{{\sbm{I}}\XS}  \def\ib{{\sbm{i}}\XS}
\def\Jb{{\sbm{J}}\XS}  \def\jb{{\sbm{j}}\XS}
\def\Kb{{\sbm{K}}\XS}  \def\kb{{\sbm{k}}\XS}
\def\Lb{{\sbm{L}}\XS}  \def\lb{{\sbm{l}}\XS}
\def\Mb{{\sbm{M}}\XS}  \def\mb{{\sbm{m}}\XS}
\def\Nb{{\sbm{N}}\XS}  \def\nb{{\sbm{n}}\XS}
\def\Ob{{\sbm{O}}\XS}  \def\ob{{\sbm{o}}\XS}
\def\Pb{{\sbm{P}}\XS}  \def\pb{{\sbm{p}}\XS}
\def\Qb{{\sbm{Q}}\XS}  \def\qb{{\sbm{q}}\XS}
\def\Rb{{\sbm{R}}\XS}  \def\rb{{\sbm{r}}\XS}
\def\Sb{{\sbm{S}}\XS}  \def\sb{{\sbm{s}}\XS}
\def\Tb{{\sbm{T}}\XS}  \def\tb{{\sbm{t}}\XS}
\def\Ub{{\sbm{U}}\XS}  \def\ub{{\sbm{u}}\XS}
\def\Vb{{\sbm{V}}\XS}  \def\vb{{\sbm{v}}\XS}
\def\Wb{{\sbm{W}}\XS}  \def\wb{{\sbm{w}}\XS}
\def\Xb{{\sbm{X}}\XS}  \def\xb{{\sbm{x}}\XS}
\def\Yb{{\sbm{Y}}\XS}  \def\yb{{\sbm{y}}\XS}
\def\Zb{{\sbm{Z}}\XS}  \def\zb{{\sbm{z}}\XS}


% ALPHABET CURSIF MAJUSCULE, taille adaptative
% Cursif,               % Cursif gras

\def\Ac{{\scu{A}}\XS}   \def\Acb{{\scb{A}}\XS}
\def\Bc{{\scu{B}}\XS}   \def\Bcb{{\scb{B}}\XS}
\def\Cc{{\scu{C}}\XS}   \def\Ccb{{\scb{C}}\XS}
\def\Dc{{\scu{D}}\XS}   \def\Dcb{{\scb{D}}\XS}
\def\Ec{{\scu{E}}\XS}   \def\Ecb{{\scb{E}}\XS}
\def\Fc{{\scu{F}}\XS}   \def\Fcb{{\scb{F}}\XS}
\def\Gc{{\scu{G}}\XS}   \def\Gcb{{\scb{G}}\XS}
\def\Hc{{\scu{H}}\XS}   \def\Hcb{{\scb{H}}\XS}
\def\Ic{{\scu{I}}\XS}   \def\Icb{{\scb{I}}\XS}
\def\Jc{{\scu{J}}\XS}   \def\Jcb{{\scb{J}}\XS}
\def\Kc{{\scu{K}}\XS}   \def\Kcb{{\scb{K}}\XS}
\def\Lc{{\scu{L}}\XS}   \def\Lcb{{\scb{L}}\XS}
\def\Mc{{\scu{M}}\XS}   \def\Mcb{{\scb{M}}\XS}
\def\Nc{{\scu{N}}\XS}   \def\Ncb{{\scb{N}}\XS}
\def\Oc{{\scu{O}}\XS}   \def\Ocb{{\scb{O}}\XS}
\def\Pc{{\scu{P}}\XS}   \def\Pcb{{\scb{P}}\XS}
\def\Qc{{\scu{Q}}\XS}   \def\Qcb{{\scb{Q}}\XS}
\def\Rc{{\scu{R}}\XS}   \def\Rcb{{\scb{R}}\XS}
\def\Sc{{\scu{S}}\XS}   \def\Scb{{\scb{S}}\XS}
\def\Tc{{\scu{T}}\XS}   \def\Tcb{{\scb{T}}\XS}
\def\Uc{{\scu{U}}\XS}   \def\Ucb{{\scb{U}}\XS}
\def\Vc{{\scu{V}}\XS}   \def\Vcb{{\scb{V}}\XS}
\def\Wc{{\scu{W}}\XS}   \def\Wcb{{\scb{W}}\XS}
\def\Xc{{\scu{X}}\XS}   \def\Xcb{{\scb{X}}\XS}
\def\Yc{{\scu{Y}}\XS}   \def\Ycb{{\scb{Y}}\XS}
\def\Zc{{\scu{Z}}\XS}   \def\Zcb{{\scb{Z}}\XS}


% ALPHABET DROIT EN MATHS, taille adaptative

\def\AD{{\sdm{A}}\XS}  \def\aD{{\sdm{a}}\XS}
\def\BD{{\sdm{B}}\XS}  \def\bD{{\sdm{b}}\XS}
\def\CD{{\sdm{C}}\XS}  \def\cD{{\sdm{c}}\XS}
\def\DD{{\sdm{D}}\XS}  \def\dD{{\sdm{d}}\XS}
\def\ED{{\sdm{E}}\XS}  \def\eD{{\sdm{e}}\XS}
\def\FD{{\sdm{F}}\XS}  \def\fD{{\sdm{f}}\XS}
\def\GD{{\sdm{G}}\XS}  \def\gD{{\sdm{g}}\XS}
\def\HD{{\sdm{H}}\XS}  \def\hD{{\sdm{h}}\XS}
\def\ID{{\sdm{I}}\XS}  \def\iD{{\sdm{i}}\XS}
\def\JD{{\sdm{J}}\XS}  \def\jD{{\sdm{j}}\XS}
\def\KD{{\sdm{K}}\XS}  \def\kD{{\sdm{k}}\XS}
\def\LD{{\sdm{L}}\XS}  \def\lD{{\sdm{l}}\XS}
\def\MD{{\sdm{M}}\XS}  \def\mD{{\sdm{m}}\XS}
\def\ND{{\sdm{N}}\XS}  \def\nD{{\sdm{n}}\XS}
\def\OD{{\sdm{O}}\XS}  \def\oD{{\sdm{o}}\XS}
\def\PD{{\sdm{P}}\XS}  \def\pD{{\sdm{p}}\XS}
\def\QD{{\sdm{Q}}\XS}  \def\qD{{\sdm{q}}\XS}
\def\RD{{\sdm{R}}\XS}  \def\rD{{\sdm{r}}\XS}
\def\SD{{\sdm{S}}\XS}  \def\sD{{\sdm{s}}\XS}
\def\TD{{\sdm{T}}\XS}  \def\tD{{\sdm{t}}\XS}
\def\UD{{\sdm{U}}\XS}  \def\uD{{\sdm{u}}\XS}
\def\VD{{\sdm{V}}\XS}  \def\vD{{\sdm{v}}\XS}
\def\WD{{\sdm{W}}\XS}  \def\wD{{\sdm{w}}\XS}
\def\XD{{\sdm{X}}\XS}  \def\xD{{\sdm{x}}\XS}
\def\YD{{\sdm{Y}}\XS}  \def\yD{{\sdm{y}}\XS}
\def\ZD{{\sdm{Z}}\XS}  \def\zD{{\sdm{z}}\XS}


% ALPHABET GRAS DROIT, taille adaptative

\def\Av{{\sbv{A}}\XS}  \def\av{{\sbv{a}}\XS}
\def\Bv{{\sbv{B}}\XS}  \def\bv{{\sbv{b}}\XS}
\def\Cv{{\sbv{C}}\XS}  \def\cv{{\sbv{c}}\XS}
\def\Dv{{\sbv{D}}\XS}  \def\dv{{\sbv{d}}\XS}
\def\Ev{{\sbv{E}}\XS}  \def\ev{{\sbv{e}}\XS}
\def\Fv{{\sbv{F}}\XS}  \def\fv{{\sbv{f}}\XS}
\def\Gv{{\sbv{G}}\XS}  \def\gv{{\sbv{g}}\XS}
\def\Hv{{\sbv{H}}\XS}  \def\hv{{\sbv{h}}\XS}
\def\Iv{{\sbv{I}}\XS}  \def\iv{{\sbv{i}}\XS}
\def\Jv{{\sbv{J}}\XS}  \def\jv{{\sbv{j}}\XS}
\def\Kv{{\sbv{K}}\XS}  \def\kv{{\sbv{k}}\XS}
\def\Lv{{\sbv{L}}\XS}  \def\lv{{\sbv{l}}\XS}
\def\Mv{{\sbv{M}}\XS}  \def\mv{{\sbv{m}}\XS}
\def\Nv{{\sbv{N}}\XS}  \def\nv{{\sbv{n}}\XS}
\def\Ov{{\sbv{O}}\XS}  \def\ov{{\sbv{o}}\XS}
\def\Pv{{\sbv{P}}\XS}  \def\pv{{\sbv{p}}\XS}
\def\Qv{{\sbv{Q}}\XS}  \def\qv{{\sbv{q}}\XS}
\def\Rv{{\sbv{R}}\XS}  \def\rv{{\sbv{r}}\XS}
\def\Sv{{\sbv{S}}\XS}  \def\sv{{\sbv{s}}\XS}
\def\Tv{{\sbv{T}}\XS}  \def\tv{{\sbv{t}}\XS}
\def\Uv{{\sbv{U}}\XS}  \def\uv{{\sbv{u}}\XS}
\def\Vv{{\sbv{V}}\XS}  \def\vv{{\sbv{v}}\XS}
\def\Wv{{\sbv{W}}\XS}  \def\wv{{\sbv{w}}\XS}
\def\Xv{{\sbv{X}}\XS}  \def\xv{{\sbv{x}}\XS}
\def\Yv{{\sbv{Y}}\XS}  \def\yv{{\sbv{y}}\XS}
\def\Zv{{\sbv{Z}}\XS}  \def\zv{{\sbv{z}}\XS}


% Nouveau (08/99) : ALPHABET BLACKBOARD, taille adaptative

\def\Abb{{\sbl{A}}\XS}  \def\abb{{\sbl{a}}\XS}
\def\Bbb{{\sbl{B}}\XS}  \def\bbb{{\sbl{b}}\XS}
\def\Cbb{{\sbl{C}}\XS}  \def\cbb{{\sbl{c}}\XS}
\def\Dbb{{\sbl{D}}\XS}  \def\dbb{{\sbl{d}}\XS}
\def\Ebb{{\sbl{E}}\XS}  \def\ebb{{\sbl{e}}\XS}
\def\Fbb{{\sbl{F}}\XS}  \def\fbb{{\sbl{f}}\XS}
\def\Gbb{{\sbl{G}}\XS}  \def\gbb{{\sbl{g}}\XS}
\def\Hbb{{\sbl{H}}\XS}  \def\hbb{{\sbl{h}}\XS}
\def\Ibb{{\sbl{I}}\XS}  \def\ibb{{\sbl{i}}\XS}
\def\Jbb{{\sbl{J}}\XS}  \def\jbb{{\sbl{j}}\XS}
\def\Kbb{{\sbl{K}}\XS}  \def\kbb{{\sbl{k}}\XS}
\def\Lbb{{\sbl{L}}\XS}  \def\lbb{{\sbl{l}}\XS}
\def\Mbb{{\sbl{M}}\XS}  \def\mbb{{\sbl{m}}\XS}
\def\Nbb{{\sbl{N}}\XS}  \def\nbb{{\sbl{n}}\XS}
\def\Obb{{\sbl{O}}\XS}  \def\obb{{\sbl{o}}\XS}
\def\Pbb{{\sbl{P}}\XS}  \def\pbb{{\sbl{p}}\XS}
\def\Qbb{{\sbl{Q}}\XS}  \def\qbb{{\sbl{q}}\XS}
\def\Rbb{{\sbl{R}}\XS}  \def\rbb{{\sbl{r}}\XS}
\def\Sbb{{\sbl{S}}\XS}  \def\sbb{{\sbl{s}}\XS}
\def\Tbb{{\sbl{T}}\XS}  \def\tbb{{\sbl{t}}\XS}
\def\Ubb{{\sbl{U}}\XS}  \def\ubb{{\sbl{u}}\XS}
\def\Vbb{{\sbl{V}}\XS}  \def\vbb{{\sbl{v}}\XS}
\def\Wbb{{\sbl{W}}\XS}  \def\wbb{{\sbl{w}}\XS}
\def\Xbb{{\sbl{X}}\XS}  \def\xbb{{\sbl{x}}\XS}
\def\Ybb{{\sbl{Y}}\XS}  \def\ybb{{\sbl{y}}\XS}
\def\Zbb{{\sbl{Z}}\XS}  \def\zbb{{\sbl{z}}\XS}

% ALPHABET GREC GRAS italique, taille adaptative

\def\alphab      {{\sbmm{\alpha}}\XS}
\def\betab       {{\sbmm{\beta}}\XS}
\def\gammab      {{\sbmm{\gamma}}\XS}      \def\Gammab    {{\sbmm{\Gamma}}\XS}
\def\deltab      {{\sbmm{\delta}}\XS}      \def\Deltab    {{\sbmm{\Delta}}\XS}
\def\epsilonb    {{\sbmm{\epsilon}}\XS}
\def\varepsilonb {{\sbmm{\varepsilon}}\XS}
\def\etab        {{\sbmm{\eta}}\XS}
\def\thetab      {{\sbmm{\theta}}\XS}      \def\Thetab    {{\sbmm{\Theta}}\XS}
\def\varthetab   {{\sbmm{\vartheta}}\XS}
\def\iotab       {{\sbmm{\iota}}\XS}
\def\kappab      {{\sbmm{\kappa}}\XS}
\def\varkappab   {{\sbmm{\varkappa}}\XS}
\def\lambdab     {{\sbmm{\lambda}}\XS}     \def\Lambdab   {{\sbmm{\Lambda}}\XS}
\def\mub         {{\sbmm{\mu}}\XS}
\def\nub         {{\sbmm{\nu}}\XS}
\def\xib         {{\sbmm{\xi}}\XS}         \def\Xib       {{\sbmm{\Xi}}\XS}
\def\pib         {{\sbmm{\pi}}\XS}         \def\Pib       {{\sbmm{\Pi}}\XS}
\def\varpib      {{\sbmm{\varpi}}\XS}
\def\rhob        {{\sbmm{\rho}}\XS}
\def\varrhob     {{\sbmm{\varrho}}\XS}
\def\sigmab      {{\sbmm{\sigma}}\XS}      \def\Sigmab    {{\sbmm{\Sigma}}\XS}
\def\varsigmab   {{\sbmm{\varsigma}}\XS}   \def\Varsigmab {{\sbmm{\Varsigma}}\XS}
\def\phib        {{\sbmm{\phi}}\XS}        \def\Phib      {{\sbmm{\Phi}}\XS}
\def\varphib     {{\sbmm{\varphi}}\XS}
\def\chib        {{\sbmm{\chi}}\XS}
\def\psib        {{\sbmm{\psi}}\XS}        \def\Psib      {{\sbmm{\Psi}}\XS}
\def\omegab      {{\sbmm{\omega}}\XS}      \def\Omegab    {{\sbmm{\Omega}}\XS}
\def\taub        {{\sbmm{\tau}}\XS}
\def\upsilonb    {{\sbmm{\upsilon}}\XS}   \def\Upsilonb  {{\sbmm{\Upsilon}}\XS}
\def\zetab       {{\sbmm{\zeta}}\XS}

\def\ellb{{\sbmm{\ell}}\XS}


% CHIFFRES
% Gras et Blackboard, taille adaptative

\def\zerob   {{\sbv{0}}\XS}        \def\zerobb   {{\sbl{O}}\XS}
\def\unb     {{\sbv{1}}\XS}        \def\unbb     {{\sbl{1}}\XS}
\def\deuxb   {{\sbv{2}}\XS}        \def\deuxbb   {{\sbl{2}}\XS}
\def\troisb  {{\sbv{3}}\XS}        \def\troisbb  {{\sbl{3}}\XS}
\def\quatreb {{\sbv{4}}\XS}        \def\quatrebb {{\sbl{4}}\XS}
\def\cinqb   {{\sbv{5}}\XS}        \def\cinqbb   {{\sbl{5}}\XS}
\def\sixb    {{\sbv{6}}\XS}        \def\sixbb    {{\sbl{6}}\XS}
\def\septb   {{\sbv{7}}\XS}        \def\septbb   {{\sbl{7}}\XS}
\def\huitb   {{\sbv{8}}\XS}        \def\huitbb   {{\sbl{8}}\XS}
\def\neufb   {{\sbv{9}}\XS}        \def\neufbb   {{\sbl{9}}\XS}


% QUELQUES ENSEMBLES

\def\eC{\Cbb}
\def\eE{\Ebb}
\def\eN{\Nbb}
\def\eQ{\Qbb}
\def\eR{\Rbb}
\def\eZ{\Zbb}
\def\eK{\Kbb}

% ALPHABET GOTHIQUES  04.06.2003  M.M. ICHIR

\def\Ag{{\textgoth{A}}\XS}  \def\ag{{\textgoth{a}}\XS}
\def\Bg{{\textgoth{B}}\XS}  \def\bg{{\textgoth{b}}\XS}
\def\Cg{{\textgoth{C}}\XS}  \def\cg{{\textgoth{c}}\XS}
\def\Dg{{\textgoth{D}}\XS}  \def\dg{{\textgoth{d}}\XS}
\def\Eg{{\textgoth{E}}\XS}  \def\eg{{\textgoth{e}}\XS}
\def\Fg{{\textgoth{F}}\XS}  \def\fg{{\textgoth{f}}\XS}
\def\Gg{{\textgoth{G}}\XS}  %\def\gg{{\textgoth{g}}\XS}
\def\Hg{{\textgoth{H}}\XS}  \def\hg{{\textgoth{h}}\XS}
\def\Ig{{\textgoth{I}}\XS}  \def\ig{{\textgoth{i}}\XS}
\def\Jg{{\textgoth{J}}\XS}  \def\jg{{\textgoth{j}}\XS}
\def\Kg{{\textgoth{K}}\XS}  \def\kg{{\textgoth{k}}\XS}
\def\Lg{{\textgoth{L}}\XS}  \def\lg{{\textgoth{l}}\XS}
\def\Mg{{\textgoth{M}}\XS}  \def\mg{{\textgoth{m}}\XS}
\def\Ng{{\textgoth{N}}\XS}  \def\ng{{\textgoth{n}}\XS}
\def\Og{{\textgoth{O}}\XS}  \def\og{{\textgoth{o}}\XS}
\def\Pg{{\textgoth{P}}\XS}  \def\pg{{\textgoth{p}}\XS}
\def\Qg{{\textgoth{Q}}\XS}  \def\qg{{\textgoth{q}}\XS}
\def\Rg{{\textgoth{R}}\XS}  \def\rg{{\textgoth{r}}\XS}
\def\Sg{{\textgoth{S}}\XS}  \def\sg{{\textgoth{s}}\XS}
\def\Tg{{\textgoth{T}}\XS}  \def\tg{{\textgoth{t}}\XS}
\def\Ug{{\textgoth{U}}\XS}  \def\ug{{\textgoth{u}}\XS}
\def\Vg{{\textgoth{V}}\XS}  \def\vg{{\textgoth{v}}\XS}
\def\Wg{{\textgoth{W}}\XS}  \def\wg{{\textgoth{w}}\XS}
\def\Xg{{\textgoth{X}}\XS}  \def\xg{{\textgoth{x}}\XS}
\def\Yg{{\textgoth{Y}}\XS}  \def\yg{{\textgoth{y}}\XS}
\def\Zg{{\textgoth{Z}}\XS}  \def\zg{{\textgoth{z}}\XS}


==> defgio.tex <==
% Fichier : defgio.tex														Auteur : Gio
% Format LaTeX2e - Linux													Date : août 99
%
% Dernière mise à jour : septembre 99
%

\typeout{\space}
\typeout{\space\space\space\space Fichier 'defgio.tex' -- JFG}
\typeout{\space}


%%%%%%%%%%%%%%%% DIVERS %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Fonction dimension texte
	\def\dimtext#1#2#3#4#5#6#7#8#9{
	\setlength{\textwidth}{#1}
	\setlength{\textheight}{#2}
	\setlength{\oddsidemargin}{#3}
	\setlength{\evensidemargin}{#4}
	\setlength{\topmargin}{#5}
	\setlength{\headheight}{#6}
	\setlength{\headsep}{#7}
	\setlength{\voffset}{#8}
	\setlength{\hoffset}{#9}
	}

% Francs, ième, BP, RIB, ...
	\def\Fcs{$^{\rm \,F}$\XS}
	\def\rib{\textsc{rib}\XS}

% Définition d'un trait
	\def\Trait{\cl{\rule{2cm}{0.02cm}}}
	%\def\Trait{\cl{\makebox[2cm][c]{\hrulefill}}\vspace*{0.5cm}}
	%\def\Trait{\cl{----------}}
	%\def\Trait#1{\cl{\rule{2cm}{0.02cm}}\vspace*{#1}}

% Quelques raccourcis perso
	\def\frem{\hfill$\triangle$}

% Divers format, taille, ...
   \def\dspsty{\displaystyle}
   \def\dispsty{\displaystyle}
   \def\sss{\scriptscriptstyle}

% Tournez SVP
	\def\TSVP{
	\vfill
	\begin{flushright}
	\dots/\dots
	\end{flushright}
	\pagebreak
	}

% Signature
	\def\Signature{
	\vfill
	\begin{small}
	\begin{flushright}
	\JFG \\
	Le \today
	\end{flushright}
	\end{small}
	}

% Mail et téléphone perso
   %\def\JFGemail{\texttt{\footnotesize Giova@IMS-Bordeaux.fr}}
   %\def\JFGemail{\texttt{\small Giova@IMS-Bordeaux.fr}}
   \def\JFGemail{\texttt{Giova@IMS-Bordeaux.fr}}
   \def\JFGtel{05 4000 3176}

% Nouveauté
	\def\bhipro{\textsc{bhi-pro}\XS}
%%%%%%%%%%%%%%%% MATHÉMATIQUE %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Garder : 
	\def\TFde#1{\Fc\cro{#1}\XS}
	%\def\DSP{densité spectrale de puissance\XS}


% Définitions pour TF, TL, TZ (A virer bientôt).
	%\def\TFde#1{\Fc\cro{#1}\XS}
	%\def\TLde#1{\Lc\cro{#1}\XS}
	%\def\TZde#1{\Zc\cro{#1}\XS}

% Divers (A virer bientôt).
	%\def\VA{variable aléatoire\XS}
	%\def\VAs{variables aléatoires\XS}
	%\def\DSP{densité spectrale de puissance\XS}
	%\def\TDS{traitement du signal\XS}    \def\GTDS{Traitement du signal\XS}
	%\def\CND{contrôle non-destructif\XS} \def\GCND{Contrôle non-destructif\XS}
   %\def\crec{chargé de recherche\XS}    \def\Crec{Chargé de recherche\XS}
   %\def\dr{directeur de recherche\XS}   \def\Dr{Directeur de recherche\XS}

% Divers à conserver
   \def\TF{transformée de Fourier\XS}   \def\GTF{Transformée de Fourier\XS}
   \def\SF{série de Fourier\XS}  		 \def\GSF{Série de Fourier\XS}  
   \def\TL{transformée de Laplace\XS}   \def\GTL{Transformée de Laplace\XS}
   \def\TZ{transformée en $z$\XS}		 \def\GTZ{Transformée en $z$\XS}
   \def\TpsC{temps continu\XS}			 \def\GTpsC{Temps continu\XS}
   \def\GTpsD{Temps discret\XS}  		 \def\TpsD{temps discret\XS}
   \def\RdC{région de convergence\XS}   \def\GRdC{Région de convergence\XS}

%%%%%%%%%%%%%%%% INFO-LANGAGE %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Matlab, octave,,scilab
	\def\mtlb{\textsl{matlab}\XS}
	\def\Mtlb{\textsl{Matlab}\XS}
	\def\octv{\textsl{octave}\XS}
	\def\Octv{\textsl{Octave}\XS}
	\def\mtlboctv{\textsl{matlab~/~octave}\XS}
	\def\MtlbOctv{\textsl{matlab~/~octave}\XS}

% Définition pour programmes Unix, ...
%
% Utilisez plutôt \usepackage{mcode}...
%
	\def\msa{\medskipamount}
	%
	\def\Prog#1{
	%
	\texttt{ 
	\indent\indent\indent
	\begin{minipage}{20cm}
	\begin{tabbing} 
	~~~~~~~ \= ~~~~~~~ \= ~~~~~~~ \= ~~~~~~~ \= ~~~~~~~\= ~~~~~~~ \= ~~~~~~~ \= ~~~~~~~ \= ~~~~~~~\=
	\\
	#1
	\end{tabbing}
	\end{minipage}
	}	% Fin de \sf
	%
	}	% Fin de définition de Prog


% ---------------------------------------------------- 
% Entête Lettre IMS à la Gio
% ---------------------------------------------------- 
%
\definecolor{BleuIMS}{cmyk}{1,1,0,0.3}	% Sur la base de CyanMagentaYellow + Black
%
\def\EnteteIMS{ 
%
\bcc\btabu{c}
%
\includegraphics[width=3cm]{LogoIMS.jpg}\\
%
{\small\color{BleuIMS} Laboratoire de l'Intégration du Matériau au Système \cnrs \umr~{\scriptsize 5218}}\\
%
{\small\color{BleuIMS} Département \laps}\\
%
{\small\color{BleuIMS} Automatique~--~Productique~--~Signal}\\
%
\etabu\ecc
}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Adresse zé tutelles

%  Equipe Signal et Image -- LAPS / IMS
%  Batiment A4 -- 6ième étage -- Bureau 625
%  351 Cours de la Libération
%  33405 TALENCE CEDEX

% Supélec et LSS
   %\def\GsY{Gif--sur--Yvette\XS}
   \newcommand{\ESE}[1][\scad]{{Supélec}\XS}
   %\def\adrshort{\ESE, Plateau de Moulon, 91192 Gif--sur--Yvette Cedex\XS}
   %\def\adresse{\ESE, Plateau de Moulon, 91192 Gif--sur--Yvette Cedex, France\XS}

   \newcommand{\adresseLSS}[1][\scad]{\ESE[#1], Plateau de Moulon, 91192 Gif--sur--Yvette Cedex, France\XS}
   \newcommand{\adresseIAS}[1][\scad]{\UPS[#1], Bât. 121, 91405 Orsay, France\XS}
   \newcommand{\adresseIMS}[1][\scad]{351 Cours de la Lib\'eration, 33405 Talence Cedex, France\XS}

   \newcommand{\tutelleLSS}[1][\scad]{\cnrs[#1]~--~\ESE[#1]~--~\ups[#1]}
   %\newcommand{\tutelleIMS}[1][\scad]{\UBI~--~\cnrs[#1]~--~\ipb[#1]}
   \newcommand{\tutelleIMS}[1][\scad]{\UdB~--~\cnrs[#1]}
   %\newcommand{\tutelleIMSBis}[1][\scad]{\cnrs[#1]~--~\ubI~--~\ipb[#1]}
   \newcommand{\tutelleIAS}[1][\scad]{\cnrs[#1]~--~\ups[#1]}

   %\def\ALSS{\LSS~(\tutelleLSS)\\\adresselss}
   %\def\ALSSun{\LSS (\tutelleLSS) \adresselss}
   %\def\AIAS{\IAS~(\tutelleIAS)\\ \adresseIAS}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


%%%%%%%%%%%%%%%% Entêtes %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Définition UPS -- Orsay
	\def\UPSCdO{
	\begin{small}
	\begin{tabular}{c} 
	\UPS	\\ 
	Faculté d'Orsay	\\ 
	-----	\\ \\ \\
	\end{tabular} 
	\end{small}
	}

% Définition UBI -- Physique
	\def\UBIPhys{
	\begin{small}
	\begin{tabular}{c} 
	\UBI	\\ 
	\ufr de physique	\\ 
	-----	\\ \\ \\
	\end{tabular} 
	\end{small}
	}

% Définition UBI -- MathInfo
	\def\UBIMathInfo{
	\begin{small}
	\begin{tabular}{c} 
	\UBI	\\ 
	\ufr de Math-Info\\ 
	-----	\\ \\ \\
	\end{tabular} 
	\end{small}
	}

% Définition UBI -- MathInfo
	\def\UBIPhysMathInfo{
	\begin{small}
	\begin{tabular}{c} 
	\UBI	\\ 
	\ufr de Physique et de Math-Info\\ 
	--------	\\ \\ \\
	\end{tabular} 
	\end{small}
	}

% Définition pour "filière" et année universitaire
	\def\Filiere#1{
	\begin{small}
	\begin{tabular}{c} 
	#1						\\ 
	Année 2012-2013	\\ 
	--------					\\ \\ \\
	\end{tabular} 
	\end{small}
	}

% Définition pour Logo UPS
	\def\LogoUPS{\includegraphics[height=1.25cm,bb=0 421 596 842]{LogoCdO}}

% Définition entête UPS
   \def\HeadUPS#1{
	\noindent
	\bcc
	\begin{tabular*}{\textwidth}{l@{\extracolsep\fill}r} 
	\UPSCdO	& \Filiere{#1}	\\ 
	\end{tabular*} 

	\vspace*{-2.5cm}
	\LogoUPS
	\ecc
   }


